PUSHing Core-Collapse Supernovae to Explosions in Spherical Symmetry II: Explodability and Global Properties

In a previously presented proof-of-principle study we established a parametrized spherically symmetric explosion method (PUSH) that can reproduce many features of core-collapse supernovae. The present paper goes beyond a specific application that is able to reproduce observational properties of SN1987A and performs a systematic study of the explosion properties for an extensive set of non-rotating, solar metallicity stellar progenitor models in the mass range from 10.8 to 120 M$_\odot$.This includes the transition from neutron stars to black holes as the final result of the collapse of massive stars, and the relation of the latter to supernovae and faint/failed supernovae. The present paper provides the basis for extended nucleosynthesis predictions in a forthcoming paper to be employed in galactic evolution models.

==> s02_explproperties_table.tex <==

\begin{center}
\begin{longtable*}{lccccc}

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- WHW02 models (standard calibration)}} \label{tab:explproperties02}\\
	
\hline
\multicolumn{1}{l}{M$_{\rm ZAMS}$} & \multicolumn{1}{c}{M$_{\rm collapse}$} & \multicolumn{1}{c}{E$_{\rm expl}$}  & \multicolumn{1}{c}{t$_{\rm expl}$} & \multicolumn{1}{c}{M$_{\rm ^{56}Ni}$} &  \multicolumn{1}{c}{M$_{\rm remn}$} \\ 
\multicolumn{1}{l}{(M$_{\odot}$)}  & \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(B)} & \multicolumn{1}{c}{(s)} &  \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(M$_{\odot}$)} \\ 
\endfirsthead

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- (continued)}} \\
\hline
\multicolumn{1}{l}{M$_{\rm ZAMS}$} & \multicolumn{1}{c}{M$_{\rm collapse}$} & \multicolumn{1}{c}{E$_{\rm expl}$}  & \multicolumn{1}{c}{t$_{\rm expl}$} & \multicolumn{1}{c}{M$_{\rm ^{56}Ni}$} &  \multicolumn{1}{c}{M$_{\rm remn}$} \\ 
\multicolumn{1}{l}{(M$_{\odot}$)}  & \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(B)} & \multicolumn{1}{c}{(s)} &  \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(M$_{\odot}$)} \\ 
\hline
\endhead
\hline
\endfoot

\hline
\endlastfoot 
	

 \tableline
10.8 & 10.43 & 0.50 & 0.56 & 2.71E-02 & 1.50 \\
11.0 & 10.61 & 0.57 & 0.39 & 2.38E-02 & 1.41 \\
11.2 & 10.81 & 0.58 & 0.35 & 2.31E-02 & 1.32 \\
11.4 & 11.01 & 0.57 & 0.38 & 2.24E-02 & 1.37 \\
11.6 & 11.13 & 0.62 & 0.34 & 2.43E-02 & 1.38 \\
11.8 & 11.06 & 0.50 & 0.46 & 2.39E-02 & 1.39 \\
12.0 & 10.93 & 0.63 & 0.55 & 3.69E-02 & 1.47 \\
12.2 & 10.93 & 0.72 & 0.48 & 3.38E-02 & 1.52 \\
12.4 & 11.03 & 0.92 & 0.41 & 4.06E-02 & 1.55 \\
12.6 & 11.14 & 0.99 & 0.35 & 4.76E-02 & 1.45 \\
12.8 & 11.27 & 0.90 & 0.28 & 3.20E-02 & 1.43 \\
13.0 & 11.36 & 1.00 & 0.38 & 4.38E-02 & 1.49 \\
13.2 & 11.49 & 1.08 & 0.41 & 4.83E-02 & 1.60 \\
13.4 & 11.59 & 1.14 & 0.40 & 5.19E-02 & 1.62 \\
13.6 & 11.72 & 1.24 & 0.40 & 5.92E-02 & 1.64 \\
13.8 & 11.85 & 1.25 & 0.40 & 6.08E-02 & 1.64 \\
14.0 & 11.97 & 1.34 & 0.40 & 6.85E-02 & 1.66 \\
14.2 & 12.08 & 1.40 & 0.40 & 7.51E-02 & 1.67 \\
14.4 & 12.23 & 1.45 & 0.40 & 8.09E-02 & 1.69 \\
14.6 & 12.38 & 1.44 & 0.40 & 8.18E-02 & 1.69 \\
14.8 & 12.49 & 1.48 & 0.42 & 8.66E-02 & 1.70 \\
15.0 & 12.64 & 1.53 & 0.41 & 9.22E-02 & 1.71 \\
15.2 & 12.72 & 1.61 & 0.43 & 1.09E-01 & 1.69 \\
15.4 & 12.89 & 1.69 & 0.44 & 1.23E-01 & 1.70 \\
15.6 & 13.01 & 1.49 & 0.44 & 1.08E-01 & 1.60 \\
15.8 & 13.11 & 1.29 & 0.42 & 9.86E-02 & 1.55 \\
16.0 & 13.25 & 1.24 & 0.40 & 7.54E-02 & 1.54 \\
16.2 & 13.42 & 1.28 & 0.41 & 8.63E-02 & 1.55 \\
16.4 & 13.54 & 1.21 & 0.38 & 6.90E-02 & 1.54 \\
16.6 & 13.72 & 1.23 & 0.37 & 8.12E-02 & 1.54 \\
16.8 & 13.84 & 1.22 & 0.36 & 7.87E-02 & 1.54 \\
17.0 & 13.84 & 1.23 & 0.36 & 7.93E-02 & 1.54 \\
17.2 & 14.08 & 1.24 & 0.35 & 7.95E-02 & 1.55 \\
17.4 & 14.22 & 1.23 & 0.34 & 6.45E-02 & 1.55 \\
17.6 & 14.35 & 1.25 & 0.33 & 7.61E-02 & 1.57 \\
17.8 & 14.46 & 1.60 & 0.44 & 1.23E-01 & 1.68 \\
18.0 & 14.50 & 1.45 & 0.44 & 1.12E-01 & 1.62 \\
18.2 & 14.59 & 1.24 & 0.39 & 7.98E-02 & 1.55 \\
18.4 & 14.83 & 1.58 & 0.42 & 9.72E-02 & 1.78 \\
18.6 & 14.86 & 1.22 & 0.36 & 6.88E-02 & 1.56 \\
18.8 & 15.05 & 1.20 & 0.36 & 6.90E-02 & 1.55 \\
19.0 & 15.04 & 1.58 & 0.43 & 1.12E-01 & 1.78 \\
19.2 & 15.09 & 1.55 & 0.43 & 1.04E-01 & 1.79 \\
19.4 & 15.23 & 1.50 & 0.44 & 1.07E-01 & 1.66 \\
19.6 & 13.37 & 0.97 & 0.27 & 3.56E-02 & 1.58 \\
19.8 & 14.54 & 1.13 & 0.35 & 6.90E-02 & 1.56 \\
20.0 & 14.74 & 1.01 & 0.37 & 6.24E-02 & 1.51 \\
20.2 & 14.47 & 0.91 & 0.26 & 3.06E-02 & 1.55 \\
20.4 & 14.81 & 1.28 & 0.35 & 8.16E-02 & 1.69 \\
20.6 & 14.03 & 1.18 & 0.41 & 1.17E-01 & 1.84 \\
20.8 & 14.35 & 1.19 & 0.39 & 1.13E-01 & 1.81 \\
21.0 & 13.00 & 1.45 & 0.46 & 1.35E-01 & 1.82 \\
21.2 & 13.56 & 1.52 & 0.44 & 1.15E-01 & 1.78 \\
21.4 & 14.80 & 1.35 & 0.41 & 1.11E-01 & 1.63 \\
21.6 & 13.63 & 1.20 & 0.35 & 8.61E-02 & 1.63 \\
21.8 & 14.79 & 1.56 & 0.43 & 1.18E-01 & 1.78 \\
22.0 & 14.42 & 1.12 & 0.35 & 6.91E-02 & 1.57 \\
22.4 & 14.77 & 1.23 & 0.35 & 9.08E-02 & 1.68 \\
22.6 & 14.68 & 1.30 & 0.39 & 1.13E-01 & 1.80 \\
25.8 & 12.37 & 0.98 & 0.35 & 8.07E-02 & 1.80 \\
26.0 & 12.94 & 0.50 & 0.55 & 1.28E-01 & 1.99 \\
26.2 & 12.24 & 0.97 & 0.33 & 7.81E-02 & 1.71 \\
26.4 & 12.55 & 1.00 & 0.32 & 8.30E-02 & 1.70 \\
26.6 & 13.19 & 1.00 & 0.31 & 7.78E-02 & 1.68 \\
26.8 & 12.99 & 1.00 & 0.31 & 7.98E-02 & 1.69 \\
27.0 & 12.45 & 0.97 & 0.34 & 8.43E-02 & 1.67 \\
27.2 & 12.76 & 0.98 & 0.34 & 8.60E-02 & 1.67 \\
27.4 & 13.04 & 0.98 & 0.34 & 8.82E-02 & 1.72 \\
27.6 & 12.79 & 0.98 & 0.34 & 8.93E-02 & 1.69 \\
27.8 & 12.57 & 0.97 & 0.34 & 9.01E-02 & 1.70 \\
28.0 & 12.67 & 0.96 & 0.33 & 8.71E-02 & 1.66 \\
28.2 & 12.81 & 1.19 & 0.42 & 1.14E-01 & 1.65 \\
29.0 & 12.62 & 1.05 & 0.39 & 9.81E-02 & 1.61 \\
30.0 & 12.25 & 1.24 & 0.45 & 1.33E-01 & 1.71 \\
31.0 & 11.72 & 0.93 & 0.34 & 8.24E-02 & 1.58 \\
32.0 & 12.00 & 1.07 & 0.36 & 1.00E-01 & 1.68 \\
33.0 & 11.44 & 1.05 & 0.37 & 1.07E-01 & 1.74 \\
34.0 & 11.78 & 0.99 & 0.39 & 1.15E-01 & 1.80 \\
35.0 & 10.64 & 1.01 & 0.36 & 9.67E-02 & 1.69 \\
36.0 & 10.31 & 1.05 & 0.38 & 1.04E-01 & 1.71 \\
37.0 & 9.72  & 1.25 & 0.48 & 1.58E-01 & 1.83 \\
38.0 & 9.27  & 0.97 & 0.33 & 8.97E-02 & 1.66 \\
40.0 & 8.75  & 0.91 & 0.37 & 8.79E-02 & 1.82 \\
75.0 & 6.36  & 0.83 & 0.30 & 2.65E-02 & 1.62 \\

\end{longtable*}
\end{center}


==> w07_explproperties_table.tex <==
\begin{center}
\begin{longtable*}{lccccc}

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- WH07 models (standard calibration)}} \label{tab:explpropertiew07}\\
	
\hline
\multicolumn{1}{l}{M$_{\rm ZAMS}$} & \multicolumn{1}{c}{M$_{\rm collapse}$} & \multicolumn{1}{c}{E$_{\rm expl}$}  & \multicolumn{1}{c}{t$_{\rm expl}$} & \multicolumn{1}{c}{M$_{\rm ^{56}Ni}$} &  \multicolumn{1}{c}{M$_{\rm remn}$} \\ 
\multicolumn{1}{l}{(M$_{\odot}$)}  & \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(B)} & \multicolumn{1}{c}{(s)} &  \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(M$_{\odot}$)} \\ 
\endfirsthead

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- (continued)}} \\
\hline
\multicolumn{1}{l}{M$_{\rm ZAMS}$} & \multicolumn{1}{c}{M$_{\rm collapse}$} & \multicolumn{1}{c}{E$_{\rm expl}$}  & \multicolumn{1}{c}{t$_{\rm expl}$} & \multicolumn{1}{c}{M$_{\rm ^{56}Ni}$} &  \multicolumn{1}{c}{M$_{\rm remn}$} \\ 
\multicolumn{1}{l}{(M$_{\odot}$)}  & \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(B)} & \multicolumn{1}{c}{(s)} &  \multicolumn{1}{c}{(M$_{\odot}$)} & \multicolumn{1}{c}{(M$_{\odot}$)} \\ 
\hline
\endhead
\hline
\endfoot

\hline
\endlastfoot 
	

 \tableline
12.0  & 10.92 & 0.81 & 0.47 & 3.87E-02 & 1.51 \\
13.0  & 11.41 & 1.20 & 0.41 & 5.50E-02 & 1.61 \\
14.0  & 12.01 & 1.39 & 0.41 & 7.15E-02 & 1.68 \\
15.0  & 12.79 & 1.70 & 0.44 & 1.17E-01 & 1.69 \\
16.0  & 13.60 & 1.20 & 0.35 & 6.64E-02 & 1.52 \\
17.0  & 14.12 & 1.25 & 0.33 & 7.03E-02 & 1.56 \\
18.0  & 14.83 & 1.59 & 0.42 & 9.40E-02 & 1.78 \\
19.0  & 15.48 & 1.34 & 0.36 & 8.71E-02 & 1.66 \\
20.0  & 15.93 & 1.19 & 0.42 & 1.12E-01 & 1.85 \\
21.0  & 16.16 & 0.99 & 0.38 & 6.22E-02 & 1.52 \\
22.0  & 16.17 & 1.08 & 0.44 & 1.14E-01 & 1.88 \\
25.0  & 15.84 & 0.73 & 0.49 & 1.18E-01 & 1.94 \\
26.0  & 15.41 & 1.01 & 0.32 & 7.33E-02 & 1.72 \\
27.0  & 15.22 & 0.98 & 0.35 & 8.62E-02 & 1.74 \\
28.0  & 15.18 & 1.32 & 0.46 & 1.53E-01 & 1.73 \\
29.0  & 14.17 & 1.01 & 0.36 & 9.63E-02 & 1.66 \\
30.0  & 13.89 & 1.12 & 0.38 & 1.08E-01 & 1.75 \\
31.0  & 13.64 & 1.02 & 0.37 & 9.93E-02 & 1.72 \\
32.0  & 13.42 & 0.95 & 0.41 & 1.13E-01 & 1.81 \\
33.0  & 13.24 & 0.71 & 0.46 & 1.18E-01 & 1.89 \\
50.0  & 9.82  & 1.13 & 0.37 & 1.06E-01 & 1.73 \\
55.0  & 9.38  & 1.08 & 0.36 & 9.97E-02 & 1.67 \\
60.0  & 7.29  & 1.19 & 0.34 & 8.32E-02 & 1.61 \\
70.0  & 6.41  & 1.37 & 0.37 & 9.84E-02 & 1.74 \\
80.0  & 6.37  & 1.31 & 0.35 & 8.80E-02 & 1.68 \\
100.0 & 6.04  & 1.50 & 0.44 & 1.23E-01 & 1.82 \\
120.0 & 6.00  & 1.30 & 0.37 & 8.09E-02 & 1.62 \\


\end{longtable*}
\end{center}
